Network Momentum across Asset Classes

We investigate the concept of network momentum, a novel trading signal derived from momentum spillover across assets. Initially observed within the confines of pairwise economic and fundamental ties, such as the stock-bond connection of the same company and stocks linked through supply-demand chains, momentum spillover implies a propagation of momentum risk premium from one asset to another. The similarity of momentum risk premium, exemplified by co-movement patterns, has been spotted across multiple asset classes including commodities, equities, bonds and currencies. However, studying the network effect of momentum spillover across these classes has been challenging due to a lack of readily available common characteristics or economic ties beyond the company level. In this paper, we explore the interconnections of momentum features across a diverse range of 64 continuous future contracts spanning these four classes. We utilise a linear and interpretable graph learning model with minimal assumptions to reveal the intricacies of the momentum spillover network. By leveraging the learned networks, we construct a network momentum strategy that exhibits a Sharpe ratio of 1.5 and an annual return of 22%, after volatility scaling, from 2000 to 2022. This paper pioneers the examination of momentum spillover across multiple asset classes using only pricing data, presents a multi-asset investment strategy based on network momentum, and underscores the effectiveness of this strategy through robust empirical analysis.

==> backtest-v20230714/perf_table_raw.tex <==
\begin{table}
\centering
\footnotesize
\caption{Performance Metrics - Raw Signals}
\label{tab:bt_perf_table_raw}
\begin{tabular}{lrrrrrrrrrr}
\toprule
{}   &  ret &    vol &  sharpe &  downside deviation &  max drawdown & max drawdown duration &  sortino &  calmar & hit rate &  avg profit over loss \\
\midrule
Long Only & 0.0324 & 0.0541 &  0.5985 &              0.0386 &        0.2003 &                15.68\% &   0.8395 &  0.1568 &   53.65\% &                0.9544 \\
MACD      & 0.0247 & 0.0478 &  0.5158 &              0.0349 &        0.1208 &                25.49\% &   0.7077 &  0.1970 &   53.08\% &                0.9665 \\
LinReg    & 0.0407 & 0.0432 &  0.9434 &              0.0305 &        0.0801 &                10.85\% &   1.3338 &  0.5064 &   53.70\% &                1.0143 \\
GMOM      & 0.0705 & 0.0517 &  1.3628 &              0.0348 &        0.0707 &                 6.90\% &   2.0265 &  1.0128 &   55.15\% &                1.0239 \\
\bottomrule
\end{tabular}
\end{table}


==> backtest-v20230714/perf_table_scaled.tex <==
\begin{table}
\centering
\caption{Performance Metrics - Rescaed to 15% Target Volatility}
\label{tab:bt_perf_table_scaled}
\begin{tabular}{lrrrrrrrrrr}
\toprule
{} &    ret &    vol &  sharpe &  downside deviation &  max drawdown & max drawdown duration &  sortino &  calmar & hit rate &  avg profit over loss \\
\midrule
Long Only & 0.1084 & 0.1476 &  0.7341 &              0.0957 &        0.6331 &                15.66\% &   1.1325 &  0.1617 &   53.65\% &                0.9716 \\
MACD      & 0.1025 & 0.1467 &  0.6991 &              0.0953 &        0.3424 &                21.60\% &   1.0756 &  0.2806 &   53.08\% &                0.9900 \\
LinReg    & 0.1653 & 0.1465 &  1.1285 &              0.0937 &        0.2852 &                10.87\% &   1.7645 &  0.5859 &   53.70\% &                1.0360 \\
GMOM      & 0.2219 & 0.1468 &  1.5110 &              0.0916 &        0.1993 &                 6.90\% &   2.4218 &  1.1789 &   55.15\% &                1.0378 \\
\bottomrule
\end{tabular}
\end{table}


==> backtest-v20230714/with_combo/perf_table_raw.tex <==
\begin{table}
\centering
\caption{Performance Metrics - Raw Signals}
\label{tab:bt_perf_table_raw}
\begin{tabular}{lrrrrrrrrrr}
\toprule
{} &   ret &   vol &  sharpe &  downside deviation &  max drawdown & max drawdown duration &  sortino &  calmar & hit rate &  avg profit over loss \\
\midrule
Long Only & 0.032 & 0.054 &   0.599 &               0.039 &         0.200 &                 15.7\% &    0.840 &   0.157 &    53.6\% &                 0.954 \\
MACD      & 0.025 & 0.048 &   0.516 &               0.035 &         0.121 &                 25.5\% &    0.708 &   0.197 &    53.1\% &                 0.967 \\
LinReg    & 0.041 & 0.043 &   0.943 &               0.031 &         0.080 &                 10.9\% &    1.334 &   0.506 &    53.7\% &                 1.014 \\
GMOM      & 0.070 & 0.052 &   1.363 &               0.035 &         0.071 &                  6.9\% &    2.026 &   1.013 &    55.2\% &                 1.024 \\
RegCombo  & 0.064 & 0.046 &   1.403 &               0.030 &         0.067 &                  5.3\% &    2.131 &   0.972 &    54.6\% &                 1.054 \\
SignCombo & 0.056 & 0.043 &   1.286 &               0.031 &         0.073 &                  7.6\% &    1.814 &   0.772 &    55.2\% &                 1.014 \\
\bottomrule
\end{tabular}
\end{table}


==> backtest-v20230714/with_combo/perf_table_scaled.tex <==
\begin{table}
\centering
\caption{Performance Metrics - Rescaed to 15% Target Volatility}
\label{tab:bt_perf_table_scaled}
\begin{tabular}{lrrrrrrrrrr}
\toprule
{} &   return &   vol. &  Sharpe &  downside deviation &  max drawdown & max drawdown duration &  Sortino &  Calmar & hit rate &  avg profit over loss \\
\midrule
Long Only & 0.108 & 0.148 &   0.734 &               0.096 &         0.633 &                 15.7\% &    1.133 &   0.162 &    53.6\% &                 0.972 \\
MACD      & 0.103 & 0.147 &   0.699 &               0.095 &         0.342 &                 21.6\% &    1.076 &   0.281 &    53.1\% &                 0.990 \\
LinReg    & 0.165 & 0.146 &   1.128 &               0.094 &         0.285 &                 10.9\% &    1.764 &   0.586 &    53.7\% &                 1.036 \\
GMOM      & 0.222 & 0.147 &   1.511 &               0.092 &         0.199 &                  6.9\% &    2.422 &   1.179 &    55.2\% &                 1.038 \\
RegCombo  & 0.226 & 0.147 &   1.536 &               0.091 &         0.201 &                  5.3\% &    2.470 &   1.194 &    54.6\% &                 1.065 \\
SignCombo & 0.219 & 0.146 &   1.493 &               0.094 &         0.218 &                  7.5\% &    2.316 &   1.061 &    55.2\% &                 1.036 \\
\bottomrule
\end{tabular}
\end{table}


==> bin/2-Preliminary.tex <==
\section{Preliminary}

\subsection{Time-series Momentum Strategy}

Time-series momentum (TSMOM) is an individual stock momentum. The daily return of a multi-asset TSMOM is defined as  
\begin{equation}
\label{eq: TSMOM}
r_{t:t+1}^{\text{portfolio}} := \frac{1}{N_t}\sum_{i=1}^{N_t} x_{i,t} \frac{\sigma_{\text{tgt}}}{\sigma_{i,t}} r_{i, t:t+1}
\end{equation}%
where $N_t$ is the number of assets at day $t$, $r_{i, t:t+1}$ is the daily return of asset $i$. With the target annualised volatility $\sigma_{\text{tgt}}$, the asset return is scaled by its annualised realised volatility $\sigma_{i,t}$. Here, $\sigma_{\text{tgt}} = 0.15$ following literature standards, and $\sigma_{i,t}$ is estimated from an exponential weighted moving standard deviation with a 60-day span on daily returns. The position, or trading signal $x_{i,t} \in [-1,1]$ at day $t$ for asset $i$ specifies the strategy. \par

The crux of momentum strategies lies in the unique construction of the trading signal $x_{i,t}$. It often consists of two steps - trend estimation and position sizing. We illustrate this with the following examples. \par

\subsubsection{Model-free TSMOM}
\paragraph{Vanilla TSMOM} \citet{moskowitzTimeSeriesMomentum2012} proposed to use past 1-year asset return $r_{i, t-252:t}$ as a trend estimation, and the direction as the position $x_{i,t} = \text{sgn}(r_{i, t-252:t})$.

\paragraph{MACD} \citet{bazDissectingInvestmentStrategies2015d} constructed trend estimation using the volatility normalised moving average crossover divergence (MACD) indicators such that
\begin{align}
    & \text{MACD}(i, t, S, L) = m(i,t,S) - m(i, t, L) \\
    & \text{MACD}_{\text{norm}}(i, t, S, L) =  \frac{\text{MACD}(i, t, S, L)}{\text{std}(p_{i, t-63:t})} \\
    & y_{i,t}(S,L) =  \frac{\text{MACD}_{\text{norm}}(i, t, S, L) }{\text{std}(\text{MACD}_{\text{norm}}(i, t-252, S, L) )} \\
    & x_{i,t} = \frac{1}{3} \sum_{k=1}^3 y_{i,t}(S_k,L_k)
\end{align}%
where $(S_k, L_k) \in \{(8,24), (16, 48), (32, 96)\}$. 

\subsubsection{Machine Learning TSMOM} While Vanilla TSMOM and MACD are model-free, recent literature managed to construct TSMOM from machine learning models. The trend estimation is formulated as a supervised learning problem with input momentum features $\mathbf{u}$.
\begin{equation}
    x_{i,t} = \text{sgn}(y_{i,t}) \quad \text{and}\quad y_{i,t}=f_{\boldsymbol{\theta}}(\mathbf{u}_{i,t})
\end{equation}%
 The model specification for $f$ are diverse, and often consider with the nature of input features $\mathbf{u}$. \citet{limEnhancingTimeSeries2020} compared linear models and deep learning models such as MLP, WaveNet and LSTM using the input features such as the MACD indicators and volatility-scaled returns from diverse lookback windows. With the same input features, \citet{woodTradingMomentumTransformer2022} considered attention-based deep learning model. The coefficients $\theta$ are estimated the mean squared error to volatility-scaled return at $t+1$ is often used. 


==> bin/2b-Preliminary-NetMOM.tex <==


\subsection{Network Momentum Strategy}

A general framework of network momentum strategies first defines a \textit{network} or a \textit{graph}\footnote{In this paper, we use \textit{graph} and \textit{network} interchangeably. Also, we use \textit{neighbours} and \textit{peers} interchangeably to represent the connected assets. In literature, the connected assets are also referred as to \textit{linked} assets. The term \textit{linkage} is thus seen in literature.} to represent certain economic links between two assets. The network is mathematically modelled by a graph adjacency matrix $\mathbf{A}_t \in \mathbb{R}^{N_t \times N_t}$ between $N_t$ assets at time $t$, where the entries  $a_{ii, t} = 0$ and $a_{ij,t} \geq 0$. If $a_{ij,t} > 0$, there exists a economic link that shows certain similarity between asset $i$ and asset $j$. Some studies \cite{moskowitzIndustriesExplainMomentum1999, boniAnalystsIndustriesPrice2006} defined binary graph such that $a_{ij,t} \in \{0, 1\}$, while others \cite{cohenEconomicLinksPredictable2008b, yamamotoMomentumInformationPropagation2021, aliSharedAnalystCoverage2020} also quantified the strength of the interconnections, which is referred as to edge weights. \par

The network momentum of asset $i$ at time $t$ is defined through a simple message passing operator that takes average of trend estimation propagated from its connected assets in $\mathbf{A}$:
\begin{equation}
\label{eq: network_momentum}
     z_{i,t} = \frac{1}{|\mathcal{N}_t(i)|} \sum_{j \in \mathcal{N}_t(i)} a_{ij, t}  z_{j,t}  
\end{equation}%
where $\mathcal{N}_t(i)$ is the neighbourhood set of asset $i$ at time $t$ containing all its connected assets, and $z_{i,t} \in \{x_{i,t}, y_{i,t}\}$ for the asset $i$ at time $t$ does not contain any information from its own. The portfolio of network momentum strategy was constructed with $z_{i,t}$. \par


In literature, different economic links were explored. Some example of $\mathbf{A}$ include:
\begin{itemize}

    \item \textit{Industry Linkage}. Stocks belonging to the same industry are connected. The graph is binary and time-insensitive such that. Different industrial classification codes were applied, such as two-digit SIC \cite{moskowitzIndustriesExplainMomentum1999} and GICS \cite{boniAnalystsIndustriesPrice2006}.

    \item \textit{Industrial Segment}. A conglomerate firm contain multiple industrial segments that corresponds to standalone firms. \citet{cohenComplicatedFirms2012} predicted return of the target conglomerate from its linked standalone firms. 

    \item \textit{Supply-demand Relations}. There exists economic links between a target company and its suppliers or/and customers. \citet{cohenEconomicLinksPredictable2008b} defines a customer link for a target firm if to which it sells more then 10\% its products or services, and constructed a customer momentum portfolio by taking average on historical customer returns.  \citet{yamamotoMomentumInformationPropagation2021a} modified the binary customer link by using centrality statistics from network theory as edge weights in $\mathbf{A}$ to show the relevant importance of customers.  \citet{menzlyMarketSegmentationCrosspredictability2010} considered supplier links together with customer links, where the edge weights are defined as the flow of goods.
    
    \item \textit{Geographic Location}. Firms whose headquarters in the same location are likely to face similar economic and political environment and therefore linked \cite{parsonsGeographicLeadLagEffects2020, korniotisStateLevelBusinessCycles2013a}.

    \item \textit{Patent Similarity}. \citet{leeTechnologicalLinksPredictable2019} define the technology link between two firms if their patent portfolios across different technology classes are similar.
    
    \item \textit{Analyst co-coverage}. The two firms that are both covered by a sell-side analyst share similar economic and business fundamentals. \citet{aliSharedAnalystCoverage2020} finds that such a connected-firm momentum factor generates a monthly alpha of 1.68\% and the co-coverage network more effectively encapsulates the information contained within other links such as industry, geographic location and customer/supplier chain. 
    
\end{itemize}


==> bin/3-Proposed-old.tex <==

A general framework of network momentum strategies first defines a \textit{network} or a \textit{graph}\footnote{In this paper, we use \textit{graph} and \textit{network} interchangeably. Also, we use \textit{neighbours} and \textit{peers} interchangeably to represent the connected assets. In literature, the connected assets are also referred as to \textit{linked} assets. The term \textit{linkage} is thus seen in literature.} to represent certain economic links between two assets. The network is mathematically modelled by a graph adjacency matrix $\mathbf{A}_t \in \mathbb{R}^{N_t \times N_t}$ between $N_t$ assets at time $t$, where the entries $a_{ii, t} = 0$ and $a_{ij,t} \geq 0$. If $a_{ij,t} > 0$, there exists a economic link that shows certain similarity between asset $i$ and asset $j$. Some studies \cite{moskowitzIndustriesExplainMomentum1999, boniAnalystsIndustriesPrice2006} defined binary graph such that $a_{ij,t} \in \{0, 1\}$, while others \cite{cohenEconomicLinksPredictable2008b, yamamotoMomentumInformationPropagation2021, aliSharedAnalystCoverage2020} also quantified the strength of the interconnections, which is referred as to edge weights. Note that network momentum assumes no self-information flow such that $a_{ii, t} = 0$, which serves the purposes of strategy diversification. This also marks a difference from cross-sectional momentum. The cross-sectional momentum takes into consideration of different assets by the means of ranking their individual time-series momentum. For network momentum, it is also feasible to construct a long/short portfolio by ranking the network momentum scores \cite{}

The network momentum of asset $i$ at time $t$ is defined through a simple message passing operator that takes average of trend estimation propagated from its connected assets:
\begin{equation}
\label{eq: network_momentum}
     y_{i,t} = \frac{1}{|\mathcal{N}_t(i)|} \sum_{j \in \mathcal{N}_t(i)} a_{ij, t}  y_{j,t}  
\end{equation}%
where $\mathcal{N}_t(i)$ is the neighbourhood set of asset $i$ at time $t$ containing all its connected assets. The portfolio of network momentum strategy was constructed with $y_{i,t}$. \par

In literature, $\mathbf{A}$ is first defined.  Table is a summary of network momentum in literature. It is very hard to find those economic and fundamental linkage . Therefore, we propose to learn from historical momentum features. 

\subsection{Graph Learning for }

\subsection{Graph Machine Learning Enhanced Network Momentum}

We propose a general graph machine learning framework to construct network momentum signals from a data-driven fashion. Suppose we have access to a momentum feature matrix $\mathbf{U}_t \in \mathbb{R}^{N_t \times F}$ of $N_t$ assets with $F$ features. The row vectors $\mathbf{U}_t = [\boldsymbol{u}_{1,t}, \boldsymbol{u}_{2,t}, \dots, \boldsymbol{u}_{N_t,t}]^{T}$ corresponds to feature vector for each asset. In line with the aforementioned \textit{machine learning TSMOM}, we can cast the construction of a network momentum strategy as a supervised learning such that
\begin{equation}
    x_{i,t} = \text{sgn}(y_{i,t}) ~ \text{and} ~ y_{i,t}=f_{\boldsymbol{\theta}} \Big( \bigoplus_{j \in \mathcal{N}_t(i)} a_{ij, t} \cdot \mathbf{u}_{j,t} \Big)
\end{equation}%
where $y_{i,t}$ is the trend estimation for network momentum and $x_{i,t}$ is the stra`tegy position. Inside the model for $y_{i,t}$, $\bigoplus$ denotes a differentiable, node permutation invariant\footnote{In the context of graph machine learning (GML), node permutation invariance is the property where for a graph $\mathcal{G}$ with node set $\mathcal{N}$ and the corresponding graph $\mathcal{G}'$ from any permutation $\mathcal{P}$ of $\mathcal{N}$, the output of GML model remains the same, i.e. $f(\mathcal{G}) = f(\mathcal{G}')$} 
function for aggregating neighbourhood information, e.g. sum, mean, min or max. $\mathcal{N}_t(i)$ represents the set of neighbourhood assets of asset $i$ at time $t$. $a_{ij, t}$ is a scalar representing the similarity strength between asset $i$ and asset $j$ at time $t$. From the perspective of graph machine learning, $y_{i,t}$ is the node representation of asset $i$ at time $t$ that is learned from the topological connections. \par

\subsubsection{Model Specification}

In order to maintain the interpretability, we mainly consider linear models in this paper. Specifically, we take the mean function as the neighbourhood aggregation function $\bigoplus$. Denote $\mathbf{x}_t = [ x_{1,t}, x_{2,t}, \dots, x_{N,t}]^T$ and $\mathbf{y}_t = [ y_{1,t}, y_{2,t}, \dots, y_{N,t}]^T$. The model can be reduced to an elegant matrix form:


\begin{equation}
    (\textbf{GMOM}) \quad \mathbf{x}_t  = \text{sgn}(\mathbf{y}_{t}) ~ \text{and} ~ \mathbf{y}_{t}= (\frac{1}{K}\sum_{k=1}^K\mathbf{A}^{(k)}_t\mathbf{U}_t) \boldsymbol{\theta} + b 
\label{eq: gmom_sr}
\end{equation}%




\subsubsection{Loss Function} The coefficients $(\boldsymbol{\theta}, b)$ in the above models are estimated by minimising w.r.t the mean squared error
\begin{itemize}
    \item{Mean Squared Error (MSE)} for training GMOM:
    \begin{equation} \label{eq:loss_MSE}
        \mathcal{L}_{\text{MSE}}(\boldsymbol{\theta}, b) = \frac{1}{|\Omega|}\sum_{(i,t) \in \Omega}\big( y_{i,t} - \frac{r_{i, t:t+1}}{\sigma_{i,t}} \big)^2
    \end{equation}
\end{itemize}


\subsection{Graph Learning for Select Peers}
To determine the  



==> bin/4-Backtest-v20230627.tex <==
\section{Performance Evaluation }

\XP{This version: v20230627 - Linear Network Momentum} 
 
\subsection{Backtest Setup}
\subsubsection{Dataset}
The backtest was implemented using 64 ratio-adjusted continuous future contracts from the Pinnacle Data Crop CLC Database. These contracts mainly contain four classes of assets, that is, Commodities, Equities, Fixed Income and Currencies. The daily price data are available from 1990 to 2022, although different assets could have different time spans when the prices are available. In Appendix, Table \ref{table:universe} lists all the assets in backtest. 

\subsubsection{Features Prepossessing}  \label{sec:subsec:momentum_features} We adopted a data winsorisation strategy for momentum features in order to mitigate the influence of outliers. Specifically, each feature of each asset was capped and floored to fall within a range defined by five times its exponentially weighted moving standard deviations from its corresponding exponentially weighted moving average. This computation was carried out using a half-life of 252 days. 

\subsubsection{Graph Learning Details} 
The first step is to decide the feature matrix $\mathbf{V}$ as the input of graph learning module. We chose the same momentum features in Section \ref{sec:subsec:momentum_features} as $\mathbf{V}$. At each day, we look back $\delta$ days, where the node set of a graph is defined as the union of assets that have less than 10\% missing values in this $\delta$-day window of momentum features. Since different assets have different time periods when the prices are available, graphs could have different sizes. In generating network momentum features with proposed GMOM and L2GMOM, we combined $K = 5$ different graphs learned from  five different lookback windows such that $\delta \in \{252, 504, 756, 1008, 1260\}$.

\subsubsection{Strategy Candidates}
For comparison against traditional time-series momentum strategies, we compare the proposed strategies against the following reference benchmarks:
\begin{itemize}
    \item{\textbf{Long Only}} takes a consistent long position $x_{i,t} = 1$ with daily volatility scaling. 
    \item{\textbf{MACD}} [ref eq]
    \item{\textbf{LinReg}} stands for Linear Regression with the eight \textit{momentum features} as input, and the [ref eq] as target. 
    \item{\textbf{GLinReg}} stands for Graph Linear Regression. We learn graph separately with Eq.\eqref{eq: gl} with an optimal $\alpha$ and $\beta$ from discrete grid search, and we fit in the [req eq]. This is to demonstrate whether the performance gain is from the end-to-end learning architecture.
\end{itemize}
We name the strategies constructed from the proposed models as \textbf{GMOM} in Eq.\eqref{eq: gmom}, \textbf{GMOM\_SR} in Eq.\eqref{eq: gmom_sr}, \textbf{L2GMOM} in Eq.\eqref{eq:l2gmom} and  \textbf{L2GMOM\_SR} in Eq.\eqref{eq:l2gmom_sr}.

\subsubsection{Optimisation Details} 
The models were trained every 5 years. This process involved coefficient optimisation and hyperparameter tuning using all preprocessed data up to the point of re-calibration. Afterwards, these optimised models were used to generate trading signals for the subsequent 5 years, using out-of-sample data. To ensure an adequate number of training samples, the first backtest period comprised of 1990-1999 for training, followed by 2000-2004 for testing. Likewise, the second period included 1990-2004 for training, and then 2005-2009 for testing. Therefore, we have an aggregated 20-year out-of-sample period from 2000 to 2020. For each backtest period, the most recent 10\% of training data was set aside as a validation set for hyperparameter tuning.

For linear models like LinReg and GMOM, there are analytical solutions. For L2GMOM, GMOM\_SR, and L2GMOM\_SR, we employed stochastic gradient descent using the \texttt{Adam} optimiser in a mini-batch approach. The validation set was utilised to determine convergence, activating early stopping when the moving average validation loss failed to improve beyond a certain threshold. To reduce the randomness introduced by the \texttt{Adam} optimiser, we carried out the experiments over 5 runs with random initial values and averaged the model outputs to create an ensemble.






\subsubsection{Model Candidates}


For a fair comparisons against the time-series momentum strategies in literature, we consider the following \textbf{baselines} form the literature:
\begin{itemize}
    \item (Model-free) \textbf{Long Only} with Volatility Scaling, i.e. $x_i^{(t)} = 1$ in Eq.\eqref{eq: TSMOM}. We hold the positions on all the assets with equal weights from the scratch.
    \item (Model-free) The \textbf{Annual Return} as a vanilla momentum \citep{moskowitzTimeSeriesMomentum2012}, i.e. $x_i^{(t)} = \text{sign}(r_i^{t-252:t})$.
    \item (Model-free) \textbf{Baz MACD} \cite{bazDissectingInvestmentStrategies2015d}, averaged on three time scales $(S, L) \in \{(8,24), (16,48), (32,96)\}$.
    \item (ML) \textbf{LR}, the ordinary linear regression,  with 5 normalised returns and 3 MACD indicators as input features. The model output is the predicted normalised return of the next day. The model parameters are estimated with the mean squared error. The strategy positions $x_i^{(t)} = \text{sign(model output)}$.
  
\end{itemize}

Correspondingly, we denote \textbf{the proposed models} as follows:
\begin{itemize}

   \item (ML) \textbf{GLR}, the ordinary linear regression, but the input features are network momentum signals, aggregating from neighbors' 5 normalised returns and 3 MACD signals. The model output is the predicted normalised return of the next day. The model parameters are estimated with the mean squared error. The strategy positions $x_i^{(t)} = \text{sign(model output)}$. The network is obtained separately by solving the convex optimisation in Eq.\eqref{eq: GL_objective_matrix}.
\end{itemize}

\subsection{General Setup}
\paragraph{Model update frequency.} The models were re-calibrated every 5 years. Specifically, we adopted a (4,1)-rolling window scheme, such that we used all the in-sample date from 1990 to 1994 to estimate the parameters, and 1995 as the out-of-sample data to report the performance. This results in a full backtest period from 1995 to 2022, a total of 28 years. \par



\subsection{Portfolio Performance}

\input{backtest-v20230627/perf_table_raw}
\input{backtest-v20230627/perf_table_scaled}

\begin{figure}[h]
    \centering
    \begin{subfigure}[]{0.49\textwidth}
        \includegraphics[width=1\textwidth]{backtest-v20230627/bt_pnl_raw.png}
        \caption{Raw signals}
        \label{subfig:glr_vs_baselines}
    \end{subfigure}
    \hspace{0.1cm}
    \begin{subfigure}[]{0.49\textwidth}
        \includegraphics[width=1\textwidth]{backtest-v20230627/bt_pnl_scaled.png}
        \caption{Signals scaled to 15\% volatility target}
        \label{subfig:glr_ml_frameworks}
    \end{subfigure}
\caption{Cumulative Returns}
\label{fig:cumulative_returns}
\end{figure}


\subsection{Orthogonality Analysis}

Whether the signals are orthogonal to the existing ones.



\begin{figure}[h!]
    \centering
    \begin{subfigure}[]{0.49\textwidth}
        \includegraphics[width=1\textwidth]{backtest-v20230627/bt_corr_scaled.png}
        \caption{Return Correlations - Scaled to 15\% Volatility Target}
        \label{subfig:corr}
    \end{subfigure}
    \hspace{0.1cm}
    \begin{subfigure}[]{0.49\textwidth}
        \includegraphics[width=1\textwidth]{backtest-v20230627/sign_agreement.png}
        \caption{Sign Agreement}
        \label{subfig:sign_agreemtn}
    \end{subfigure}
\caption{Orthogonal Analysis: Correlations and Sign Agreement}
\label{fig:cumulative_returns}
\end{figure}


\subsection{Turnover Analysis}

Whether the signals make money after considering the turnover

\begin{figure}[h!]
    \centering
    \begin{subfigure}[]{0.49\textwidth}
        \includegraphics[width=1\textwidth]{backtest-v20230627/avg_turnover.png}
        \caption{Average Turnover}
        \label{subfig:corr}
    \end{subfigure}
    \hspace{0.1cm}
    \begin{subfigure}[]{0.49\textwidth}
        \includegraphics[width=1\textwidth]{backtest-v20230627/sr_turnover.png}
        \caption{Sharpe Ratio under different cost}
        \label{subfig:sign_agreemtn}
    \end{subfigure}
\caption{Turnover Analysis: \XP{The post-cost Sharpe ratio is not good. We need to use turnover regularisation. The average turnover, however, matches Bryan Lim's results.}}
\label{fig:cumulative_returns}
\end{figure}


==> bin/4-Backtest-v20230711.tex <==
\section{Empirical Analysis}

\subsection{Data}

The backtest was implemented using 64 ratio-adjusted continuous future contracts from the Pinnacle Data Crop CLC Database. These contracts contain four classes of assets, that is, Commodities, Equities, Fixed Income (FI) and Currencies (FX). The daily price data are available from 1990 to 2022, although different assets could have different spans when the prices are available. In Appendix, Table \ref{table:universe} lists all the assets used in backtest.  \par

We adopted a data winsorisation strategy for momentum features in order to mitigate the influence of outliers. Specifically, each feature of each asset was capped and floored to fall within a range defined by five times its exponentially weighted moving standard deviations from its corresponding exponentially weighted moving average. This computation was carried out using a half-life of 252 days.  \par

\subsection{Backtest Setup}

\paragraph{Graph Learning Details}
The first step is to decide the feature matrix $\mathbf{V}$ as the input of graph learning module. We chose the momentum features in Section \ref{sec:subsec:momentum_features} as $\mathbf{V}$. At each day, we look back $\delta$ days, where the node set of a graph is defined as the union of assets that have less than 10\% missing values in this $\delta$-day window of momentum features. Since different assets have different time periods when the prices are available, graphs could have different sizes. In generating network momentum features with proposed GMOM and L2GMOM, we combined $K = 5$ different graphs learned from  five different lookback windows such that $\delta \in \{252, 504, 756, 1008, 1260\}$.

\paragraph{Strategy Candidates}
For comparison against traditional time-series momentum strategies, we compare the proposed strategies against the following reference benchmarks:
\begin{itemize}
    \item{\textbf{Long Only}} takes a consistent long position $x_{i,t} = 1$ with daily volatility scaling. 
    \item{\textbf{MACD}} [ref eq]
    \item{\textbf{LinReg}} stands for Linear Regression with the eight \textit{momentum features} as input, and the [ref eq] as target. 
\end{itemize}

\paragraph{Optimisation Details}

The models were trained every 5 years. This process involved coefficient optimisation and hyperparameter tuning using all preprocessed data up to the point of re-calibration. Afterwards, these optimised models were used to generate trading signals for the subsequent 5 years, using out-of-sample data. To ensure an adequate number of training samples, the first backtest period comprised of 1990-1999 for training, followed by 2000-2004 for testing. Likewise, the second period included 1990-2004 for training, and then 2005-2009 for testing. Therefore, we have an aggregated 20-year out-of-sample period from 2000 to 2020. For each backtest period, the most recent 10\% of training data was set aside as a validation set for hyperparameter tuning.

For linear models like LinReg and GMOM, there are analytical solutions. For L2GMOM, GMOM\_SR, and L2GMOM\_SR, we employed stochastic gradient descent using the \texttt{Adam} optimiser in a mini-batch approach. The validation set was utilised to determine convergence, activating early stopping when the moving average validation loss failed to improve beyond a certain threshold. To reduce the randomness introduced by the \texttt{Adam} optimiser, we carried out the experiments over 5 runs with random initial values and averaged the model outputs to create an ensemble.



\subsection{Portfolio Performance}
\input{backtest-v20230711/perf_table_combined}

\begin{figure} 
    \centering
    \begin{subfigure}[]{0.49\textwidth}
        \includegraphics[width=1\textwidth]{backtest-v20230711/bt_pnl_raw.png}
        \caption{Raw signals}
        \label{subfig:cumulative_returns_raw}
    \end{subfigure}
    \hspace{0.1cm}
    \begin{subfigure}[]{0.49\textwidth}
        \includegraphics[width=1\textwidth]{backtest-v20230711/bt_pnl_scaled.png}
        \caption{Signals scaled to 15\% volatility target}
        \label{subfig:cumulative_returns_scaled}
    \end{subfigure}
\caption{Cumulative Returns}
\label{fig:cumulative_returns}
\end{figure}

In evaluating the portfolio performance, we use the following annualised metrics in Table \ref{tab:bt_perf_table_raw}:
\begin{itemize}
    \item{\textbf{Profitability Measures}}: expected return and hit rate (the percentage of days with positive returns across the test period)
    \item{\textbf{Risk Measures}}: daily volatility (vol.), downside deviation, maximum drawdown (MDD) and MDD duration (the percentage of days with MDD across the test period).
    \item{\textbf{Overall Performance Measures}}: Sharpe ratio (expected return$/$vol.), Sortino ratio (expected return$/$downside deviation), Calmar ratio (expected return$/$MDD), and the average profits over the average loss ($\frac{\text{Avg. P}}{\text{Avg. L}}$).
\end{itemize}%
In order to have a better comparison between different strategies, we apply an additional layer of volatility scaling at the portfolio level to an annualised volatility target of 15\% and report the above evaluation metrics. 




\subsection{Diversification Analysis}

\begin{figure}[h!]
    \centering
        \begin{subfigure}[]{0.33\textwidth}
        \includegraphics[width=1\textwidth]{backtest-v20230711/bt_corr_raw.png}
        \caption{Raw Return Correlations}
        \label{subfig:bt_corr_raw}
    \end{subfigure}%
    \begin{subfigure}[]{0.33\textwidth}
        \includegraphics[width=1\textwidth]{backtest-v20230711/bt_corr_scaled.png}
        \caption{Scaled Return Correlations}
        \label{subfig:bt_corr}
    \end{subfigure}%
    \begin{subfigure}[]{0.33\textwidth}
        \includegraphics[width=1\textwidth]{backtest-v20230711/sign_agreement.png}
        \caption{Sign Agreement}
        \label{subfig:sign_agreemtn}
    \end{subfigure}
\caption{Diversification Analysis}
\label{fig:diversification_analysis}
\end{figure}


\subsection{Turnover Analysis}

\begin{figure}[h!]
    \centering
        \begin{subfigure}[]{0.5\textwidth}
        \includegraphics[width=1\textwidth]{backtest-v20230711/avg_turnover.png}
        \caption{Average Turnover}
        \label{subfig:turnover}
    \end{subfigure}%
    \begin{subfigure}[]{0.5\textwidth}
        \includegraphics[width=1\textwidth]{backtest-v20230711/sr_turnover.png}
        \caption{Ex-cost Sharpe}
        \label{subfig:sr_turnover}
    \end{subfigure}
\caption{Turnover Analysis}
\label{fig:Turnover_analysis}
\end{figure}



==> bin/5-Robustness-v20230711.tex <==
\section{Robustness Analysis}

\subsection{Graph Topology Analysis}

% topology analysis
% should we use the ensemble edges?

\subsubsection{Community Structure}



\subsection{Portfolio of Asset Class}

% covering the inter-class edges, what are the portfolio performance whithin each class? and alpha. What are their correlation? 

% how about we only use inter-class edge?

\subsection{Momentum or Mean Revision}
% put this in journal paper. 

In GMOM and L2GMOM, we restrict the graph adjacency matrix only with non-negative entries whose value reflect the momentum spillover effects between two assets. So the graph momentum features reflect the momentum trends of target assets. However, since we applied linear model whether the coefficients are learned. Therefore, negative coefficients may contradict the basic philosophy of momentum strategy. 

In figure , we plot the change of graph momentum/momentum coefficients. 

literature?


\begin{figure}
\centering
    \includegraphics[width=0.9\textwidth]{backtest-v20230627/coef-2015.png}
    \caption{Coefficient estimation of different momentum features}
    \label{fig:coef_main_2015}
\end{figure}

\subsection{Panel Analysis}
 Construct separate portfolio with only commodity, equities, FI and FX?

==> bin/backtest-v20230627/perf_table_raw.tex <==
\begin{table}[h]
\small
\caption{Performance Metrics - Raw Signals}
\label{tab:bt_perf_table_raw}
\begin{tabular}{llllllrllrl}
\toprule
{} &    return &    vol. &  sharpe &  \makecell{downside \\ deviation} & \makecell{MDD} &  \makecell{MDD \\ duration} &  sortino &  calmar &  hit rate &  $\frac{\text{Avg. P}}{\text{Avg. L}}$ \\
\midrule
\multicolumn{11}{l}{\textbf{References:}  } \\
Long Only & 0.029 & 0.054 &   0.547 &               0.037 &         0.186 &                 16.5\% &    0.785 &   0.153 &    53.5\% &                 0.950 \\
MACD      & 0.019 & 0.036 &   0.539 &               0.027 &         0.090 &                 19.5\% &    0.733 &   0.212 &    53.1\% &                 0.971 \\
LinReg    & 0.038 & 0.043 &   0.891 &               0.030 &         0.088 &                 12.5\% &    1.270 &   0.429 &    52.8\% &                 1.040 \\

\multicolumn{11}{l}{\textbf{Trained with MSE:}  } \\
GMOM      & 0.063 & 0.051 &   1.230 &               0.034 &         0.081 &                 11.2\% &    1.842 &   0.766 &    53.4\% &                 1.014 \\
L2GMOM    & 0.065 & 0.047 &   1.391 &               0.030 &         0.066 &                  7.4\% &    2.181 &   0.967 &    52.4\% &                 1.085 \\

\multicolumn{11}{l}{\textbf{Trained with Sharpe Ratio:}  } \\
GMOM\_sr   & 0.038 & 0.031 &   1.248 &               0.021 &         0.061 &                 11.8\% &    1.787 &   0.615 &    53.1\% &                 1.035 \\
L2GMOM\_sr & 0.044 & 0.032 &   1.387 &               0.023 &         0.052 &                  6.4\% &    1.902 &   0.839 &    53.7\% &                 1.051 \\
\bottomrule
\end{tabular}
\end{table}



==> bin/backtest-v20230627/perf_table_scaled.tex <==
\begin{table}[h]
\small
\centering
\caption{Performance Metrics - Rescaled to 15\% Target Volatility}
\label{tab:bt_perf_table_scaled}
\begin{tabular}{llllllrllrl}
\toprule
{} &    return &    vol. &  sharpe &  \makecell{downside \\ deviation} & \makecell{MDD} &  \makecell{MDD \\ duration} &  sortino &  calmar &  hit rate &  $\frac{\text{Avg. P}}{\text{Avg. L}}$ \\
\midrule
\multicolumn{11}{l}{\textbf{References:}  } \\

Long Only & 0.097 & 0.147 &   0.656 &               0.095 &         0.572 &                 16.8\% &    1.013 &   0.156 &    53.5\% &                 0.964 \\
MACD      & 0.111 & 0.146 &   0.758 &               0.096 &         0.329 &                 16.5\% &    1.158 &   0.320 &    53.1\% &                 0.999 \\
LinReg    & 0.159 & 0.146 &   1.089 &               0.094 &         0.339 &                  9.7\% &    1.692 &   0.470 &    52.8\% &                 1.068 \\

\multicolumn{11}{l}{\textbf{Trained with MSE:}  } \\
GMOM      & 0.206 & 0.147 &   1.402 &               0.090 &         0.234 &                 11.8\% &    2.282 &   0.894 &    53.4\% &                 1.034 \\
L2GMOM    & 0.223 & 0.147 &   1.517 &               0.089 &         0.186 &                  7.4\% &    2.517 &   1.237 &    52.4\% &                 1.098 \\

\multicolumn{11}{l}{\textbf{Trained with Sharpe Ratio:}  } \\
GMOM\_sr   & 0.219 & 0.146 &   1.497 &               0.094 &         0.250 &                 11.8\% &    2.336 &   0.902 &    53.1\% &                 1.069 \\
L2GMOM\_sr & 0.253 & 0.146 &   1.736 &               0.094 &         0.174 &                  5.9\% &    2.707 &   1.537 &    53.7\% &                 1.091 \\
\bottomrule
\end{tabular}
\end{table}

==> bin/backtest-v20230711/perf_table_combined.tex <==
\begin{table*}[t]
\caption{Portfolio Performance Metrics}
\label{tab:bt_perf_table_raw}
\small
\begin{threeparttable}
\begin{tabular}{lllllllllll}
\toprule
{} &    return &    vol. &  sharpe &  \makecell{downside \\ deviation} & \makecell{MDD} &  \makecell{MDD \\ duration} &  sortino &  calmar &  hit rate &  $\frac{\text{Avg. P}}{\text{Avg. L}}$ \\
\midrule
\multicolumn{11}{l}{\textbf{Raw Signals:}  } \\
Long Only & 0.0294 & 0.0537 &  0.5469 &              0.0374 &        0.1855 &                16.51\% &   0.7846 &  0.1526 &   53.52\% &                0.9498 \\
MACD      & 0.0195 & 0.0361 &  0.5386 &              0.0266 &        0.0896 &                19.52\% &   0.7326 &  0.2117 &   53.09\% &                0.9705 \\
LinReg    & 0.0382 & 0.0428 &  0.8906 &              0.0300 &        0.0884 &                12.54\% &   1.2700 &  0.4292 &   52.84\% &                1.0404 \\
GMOM      & 0.0675 & 0.0503 &  1.3427 &              0.0333 &        0.0724 &                 7.46\% &   2.0250 &  0.9204 &   53.30\% &                1.0376 \\
\midrule
\multicolumn{11}{l}{\textbf{Signals Rescaled to 15\% Target Volatility:}  } \\
Long Only & 0.0966 & 0.1471 &  0.6564 &              0.0954 &        0.5719 &                16.78\% &   1.0127 &  0.1564 &   53.52\% &                0.9641 \\
MACD      & 0.1110 & 0.1464 &  0.7579 &              0.0958 &        0.3293 &                16.54\% &   1.1581 &  0.3200 &   53.09\% &                0.9992 \\
LinReg    & 0.1586 & 0.1457 &  1.0889 &              0.0938 &        0.3391 &                 9.68\% &   1.6916 &  0.4702 &   52.84\% &                1.0678 \\
GMOM      & 0.2197 & 0.1467 &  1.4983 &              0.0901 &        0.1957 &                 7.46\% &   2.4401 &  1.1543 &   53.30\% &                1.0544 \\
\bottomrule
\end{tabular}
    \begin{tablenotes}
      \item[a] Best performance of each metric is labelled with ($^\ast$) 
    \end{tablenotes}
\end{threeparttable}
\end{table*}




==> bin/backtest-v20230711/perf_table_raw.tex <==
\begin{table}
\centering
\caption{Performance Metrics - Raw Signals}
\label{tab:bt_perf_table_raw}
\begin{tabular}{lrrrrrrrrrr}
\toprule
{} &    ret &    vol &  sharpe &  downside deviation &  max drawdown & max drawdown duration &  sortino &  calmar & hit rate &  avg profit over loss \\
\midrule
Long Only & 0.0294 & 0.0537 &  0.5469 &              0.0374 &        0.1855 &                16.51\% &   0.7846 &  0.1526 &   53.52\% &                0.9498 \\
MACD      & 0.0195 & 0.0361 &  0.5386 &              0.0266 &        0.0896 &                19.52\% &   0.7326 &  0.2117 &   53.09\% &                0.9705 \\
LinReg    & 0.0382 & 0.0428 &  0.8906 &              0.0300 &        0.0884 &                12.54\% &   1.2700 &  0.4292 &   52.84\% &                1.0404 \\
GMOM      & 0.0675 & 0.0503 &  1.3427 &              0.0333 &        0.0724 &                 7.46\% &   2.0250 &  0.9204 &   53.30\% &                1.0376 \\
\bottomrule
\end{tabular}
\end{table}


==> bin/backtest-v20230711/perf_table_scaled.tex <==
\begin{table}
\centering
\caption{Performance Metrics - Rescaed to 15% Target Volatility}
\label{tab:bt_perf_table_scaled}
\begin{tabular}{lrrrrrrrrrr}
\toprule
{} &    ret &    vol &  sharpe &  downside deviation &  max drawdown & max drawdown duration &  sortino &  calmar & hit rate &  avg profit over loss \\
\midrule
Long Only & 0.0966 & 0.1471 &  0.6564 &              0.0954 &        0.5719 &                16.78\% &   1.0127 &  0.1564 &   53.52\% &                0.9641 \\
MACD      & 0.1110 & 0.1464 &  0.7579 &              0.0958 &        0.3293 &                16.54\% &   1.1581 &  0.3200 &   53.09\% &                0.9992 \\
LinReg    & 0.1586 & 0.1457 &  1.0889 &              0.0938 &        0.3391 &                 9.68\% &   1.6916 &  0.4702 &   52.84\% &                1.0678 \\
GMOM      & 0.2197 & 0.1467 &  1.4983 &              0.0901 &        0.1957 &                 7.46\% &   2.4401 &  1.1543 &   53.30\% &                1.0544 \\
\bottomrule
\end{tabular}
\end{table}


==> robustness-v20230714/lookback/perf_table_raw.tex <==
\begin{table}
\centering
\caption{Performance Metrics - Raw Signals}
\label{tab:bt_perf_table_raw}
\begin{tabular}{lrrrrrrrrrr}
\toprule
{} &   ret &   vol &  sharpe &  downside deviation &  max drawdown & max drawdown duration &  sortino &  calmar & hit rate &  avg profit over loss \\
\midrule
GMOM    & 0.066 & 0.052 &   1.277 &               0.035 &         0.073 &                  6.9\% &    1.900 &   0.912 &    54.2\% &                 1.048 \\
lb-252  & 0.058 & 0.049 &   1.185 &               0.034 &         0.085 &                  7.0\% &    1.710 &   0.697 &    54.4\% &                 1.027 \\
lb-504  & 0.057 & 0.051 &   1.128 &               0.035 &         0.080 &                  7.5\% &    1.660 &   0.718 &    53.5\% &                 1.054 \\
lb-756  & 0.058 & 0.052 &   1.126 &               0.035 &         0.086 &                  8.5\% &    1.668 &   0.678 &    54.2\% &                 1.023 \\
lb-1008 & 0.058 & 0.052 &   1.106 &               0.035 &         0.095 &                  9.6\% &    1.648 &   0.607 &    54.1\% &                 1.022 \\
lb-1260 & 0.058 & 0.052 &   1.117 &               0.035 &         0.091 &                 11.2\% &    1.671 &   0.641 &    54.2\% &                 1.018 \\
\bottomrule
\end{tabular}
\end{table}


==> robustness-v20230714/robust_table_coef.tex <==
\begin{table*}
\centering
\caption{Coefficients of Linear Models}
\label{tab:bt_perf_table_scaled}
\footnotesize
\label{tab:lr}
\begin{threeparttable}
\begin{tabular}{lllllllll}
\toprule
\makecell{in-sample \\ period}  & \makecell{vol-scaled \\ 1d ret} &  \makecell{vol-scaled \\ 1m return} & \makecell{vol-scaled \\ 3m return} & \makecell{vol-scaled \\ 6m return} & \makecell{vol-scaled \\ 1y return} & macd(8,24) &  macd(16,48) &     macd(32,96) \\
\midrule
\multicolumn{9}{c}{Panel A: LinReg}  \\
\midrule
1990-1999       &  \makecell{0.039* \\ (0.003)} &   \makecell{-0.009 \\ (0.006)} &   \makecell{0.007 \\ (0.006)} &  \makecell{-0.020* \\ (0.006)} &  \makecell{0.025* \\ (0.005)} &  \makecell{0.027* \\ (0.008)} &   \makecell{-0.011 \\ (0.006)} &  \makecell{0.006 \\ (0.004)} \\ [0.4cm]

1990-2004       &  \makecell{0.030* \\ (0.003)} &  \makecell{-0.011* \\ (0.005)} &   \makecell{0.008 \\ (0.004)} &  \makecell{-0.013* \\ (0.004)} &  \makecell{0.026* \\ (0.004)} &  \makecell{0.026* \\ (0.005)} &  \makecell{-0.017* \\ (0.004)} &  \makecell{0.009* \\ (0.002)} \\ [0.4cm]

1990-2009       &  \makecell{0.020* \\ (0.002)} &   \makecell{-0.004 \\ (0.004)} &   \makecell{0.003 \\ (0.004)} &   \makecell{-0.005 \\ (0.004)} &  \makecell{0.022* \\ (0.003)} &  \makecell{0.017* \\ (0.005)} &  \makecell{-0.013* \\ (0.004)} &  \makecell{0.006* \\ (0.002)} \\  [0.4cm]

1990-2014       &  \makecell{0.017* \\ (0.002)} &   \makecell{-0.004 \\ (0.003)} &   \makecell{0.003 \\ (0.003)} &   \makecell{-0.002 \\ (0.003)} &  \makecell{0.014* \\ (0.003)} &  \makecell{0.016* \\ (0.004)} &  \makecell{-0.010* \\ (0.003)} &  \makecell{0.006* \\ (0.002)} \\ [0.4cm]

1990-2019       &  \makecell{0.013* \\ (0.002)} &   \makecell{-0.002 \\ (0.003)} &   \makecell{0.005 \\ (0.003)} &    \makecell{0.001 \\ (0.003)} &  \makecell{0.016* \\ (0.002)} &  \makecell{0.011* \\ (0.004)} &  \makecell{-0.012* \\ (0.003)} &  \makecell{0.006* \\ (0.002)} \\

\midrule
\multicolumn{9}{c}{Panel A: GMOM}  \\
\midrule
1990-1999 & \makecell{0.068* \\ (0.010)} & \makecell{-0.028 \\ (0.019)} & \makecell{0.002 \\ (0.018)} & \makecell{-0.031 \\ (0.016)} & \makecell{0.030* \\ (0.015)} & \makecell{0.085* \\ (0.028)} & \makecell{-0.054* \\ (0.026)} & \makecell{0.028 \\ (0.015)} \\ [0.4cm]

1990-2004 & \makecell{0.090* \\ (0.008)} & \makecell{-0.055* \\ (0.015)} & \makecell{0.006 \\ (0.013)} & \makecell{-0.011 \\ (0.013)} & \makecell{0.048* \\ (0.011)} & \makecell{0.095* \\ (0.020)} & \makecell{-0.078* \\ (0.016)} & \makecell{0.028* \\ (0.008)} \\ [0.4cm]

1990-2009 & \makecell{0.070* \\ (0.006)} & \makecell{-0.041* \\ (0.012)} & \makecell{-0.022* \\ (0.011)} & \makecell{0.009 \\ (0.010)} & \makecell{0.040* \\ (0.009)} & \makecell{0.057* \\ (0.016)} & \makecell{-0.045* \\ (0.013)} & \makecell{0.017* \\ (0.007)} \\ [0.4cm]

1990-2014 & \makecell{0.073* \\ (0.005)} & \makecell{-0.034* \\ (0.009)} & \makecell{-0.025* \\ (0.008)} & \makecell{0.007 \\ (0.007)} & \makecell{-0.006 \\ (0.006)} & \makecell{0.062* \\ (0.012)} & \makecell{-0.026* \\ (0.011)} & \makecell{0.022* \\ (0.006)} \\ [0.4cm]

1990-2019 & \makecell{0.067* \\ (0.004)} & \makecell{-0.029* \\ (0.008)} & \makecell{-0.009 \\ (0.007)} & \makecell{0.017* \\ (0.007)} & \makecell{-0.002 \\ (0.005)} & \makecell{0.047* \\ (0.011)} & \makecell{-0.039* \\ (0.010)} & \makecell{0.025* \\ (0.005)} \\

\bottomrule
\end{tabular}

\begin{tablenotes}
  \item[a] Significant coefficients with $p$-value of statistic $t$ test are marked with $\ast$
\end{tablenotes}

\end{threeparttable}
\end{table*}


==> robustness-v20230714/robust_table_raw.tex <==
\begin{table}[h!]
\centering
\caption{Performance of GMOM portfolios across asset classes from raw signals}
\label{tab:robust_perf_table_raw}
  \footnotesize
\begin{threeparttable}
\begin{tabular}{lllllllllll}
\toprule
{} &    return &    vol. &  sharpe &  \makecell{downside \\ deviation} & \makecell{MDD} &  \makecell{MDD \\ duration} &  sortino &  calmar &  hit rate &  $\frac{\text{Avg. P}}{\text{Avg. L}}$ \\
\midrule
GMOM  & 0.070 & 0.052 &   1.363* &               0.035 &         0.071* &                  6.9\%* &    2.026* &   1.013* &    55.2\%* &                 1.024 \\
\midrule
\multicolumn{11}{c}{Panel A: Multi-class GMOM with Intra- or Inter-Class Edges}  \\
\midrule
GMOM-Intra & 0.051 & 0.048* &   1.050 &               0.033* &         0.079 &                  8.9\% &    1.525 &   0.639 &    54.2\% &                 1.008 \\
GMOM-Inter & 0.035 & 0.049 &   0.719 &               0.035 &         0.234 &                 27.5\% &    1.012 &   0.147 &    53.5\% &                 0.984 \\

\midrule
\multicolumn{11}{c}{Panel B: Individual Asset Class Portfolio from Multi-class GMOM} \\
\midrule
GMOM-Commd & 0.050 & 0.064 &   0.791 &               0.046 &         0.183 &                 15.0\% &    1.089 &   0.271 &    53.1\% &                 1.012 \\
GMOM-Equity & 0.101 & 0.122 &   0.826 &               0.088 &         0.250 &                 18.2\% &    1.141 &   0.391 &    54.0\% &                 0.980 \\
GMOM-FI     & 0.139* & 0.118 &   1.176 &               0.077 &         0.305 &                 13.2\% &    1.815 &   0.463 &    53.7\% &                 1.047 \\
GMOM-FX     & 0.045 & 0.070 &   0.637 &               0.046 &         0.259 &                 28.7\% &    0.973 &   0.167 &    51.8\% &                 1.034 \\
\midrule
\multicolumn{11}{c}{Panel C: Individual Asset Class Portfolio from Single-class GMOM}\\
\midrule
Commd   & 0.037 & 0.054 &   0.676 &               0.042 &         0.121 &                  9.7\% &    0.876 &   0.297 &    52.8\% &                 1.009 \\
Equity    & 0.043 & 0.125 &   0.346 &               0.086 &         0.529 &                 29.8\% &    0.500 &   0.068 &    52.1\% &                 0.974 \\
FI        & 0.093 & 0.122 &   0.768 &               0.076 &         0.331 &                 12.0\% &    1.228 &   0.271 &    51.9\% &                 1.052* \\
FX        & 0.006 & 0.068 &   0.094 &               0.046 &         0.321 &                 40.2\% &    0.139 &   0.013 &    50.9\% &                 0.979 \\
\bottomrule
\end{tabular}
    \begin{tablenotes}
      \item[a] Cross-Panel best performance of each metric is labelled with ($^\ast$) 
      \item[b] Four classes include Commodities (Commd), Equities (Equity), Fixed Income (FI) and Foreign Currencies (FX)
    \end{tablenotes}
\end{threeparttable}
\end{table}





  %\item[c] In GMOM, the graphs were derived from a set of 64 assets which were classified into the aforementioned four asset classes. In GMOM-Intra (Panel A), graph connections were restricted to only those edges that linked two assets from the same class. Conversely, in GMOM-Inter (Panel A), we only considered those edges that linked assets from different classes. Panel B lists four portfolios that filter GMOM signals for each individual class, however, information from other classes is inherently present in each class by graph connections. By contrast, Panel C lists four strategies, where we learned new graphs from assets that belong to the same class, and subsequently formed individual strategies. Therefore, the portfolios in Panel C do not contain any information of other three classes.

==> tables/literature.tex <==
\begin{table}[h!]
\centering
\scriptsize
\caption{An overview of traditional network momentum strategies.}
\begin{tabular}{@{}llll@{}}
\toprule
Literature & Network Construction & Trend Estimation & Position Sizing \\ \midrule
   \cite{ali2020shared}        &    analyst co-coverage        &    weighted average  of past-month returns    &    long top 20\%  short bottom 20\%     \\
           &                      &                  &                 \\ \bottomrule
\end{tabular}
\end{table}
